Transformers Can Do Bayesian Inference

Currently, it is hard to reap the benefits of deep learning for Bayesian methods, which allow the explicit specification of prior knowledge and accurately capture model uncertainty. We present Prior-Data Fitted Networks (PFNs). PFNs leverage in-context learning in large-scale machine learning techniques to approximate a large set of posteriors. The only requirement for PFNs to work is the ability to sample from a prior distribution over supervised learning tasks (or functions). Our method restates the objective of posterior approximation as a supervised classification problem with a set-valued input: it repeatedly draws a task (or function) from the prior, draws a set of data points and their labels from it, masks one of the labels and learns to make probabilistic predictions for it based on the set-valued input of the rest of the data points. Presented with a set of samples from a new supervised learning task as input, PFNs make probabilistic predictions for arbitrary other data points in a single forward propagation, having learned to approximate Bayesian inference. We demonstrate that PFNs can near-perfectly mimic Gaussian processes and also enable efficient Bayesian inference for intractable problems, with over 200-fold speedups in multiple setups compared to current methods. We obtain strong results in very diverse areas such as Gaussian process regression, Bayesian neural networks, classification for small tabular data sets, and few-shot image classification, demonstrating the generality of PFNs. Code and trained PFNs are released at https://github.com/automl/TransformersCanDoBayesianInference.

==> bo_for_hpo.tex <==

\subsection{Application to BO for HPO}


In this section, we want to evaluate how PFNs can be used to perform Bayesian Optimization (BO). BO is a method for Hyperparameter Optimization (HPO), where the objective is to find the best hyperparameter configuration $x \in \mathcal{X}$ that minimize a function $f: \mathcal{X} \rightarrow\mathbb{R} $. To optimize the function, BO relies on a probabilistic model $s(\mathbf{x})$, or surrogate, that approximates the function $f$. Given a history of observations $\mathcal{D} = \{(\mathbf{x}_i, y_i)\}^N_i$, the surrogate model provides uncertainty estimations over the domain of $f$, which are used to query the next hyperparameter $x_*$ by maximizing an acquisition function $a(\mathbf{x}|\mathcal{D})$. BO alternates the update of the surrogate and the selection of the next configuration.

A typical choice for surrogate is a Gaussian Process (GP) \citep{rasmussen-book06a}, whose posterior can be computed analitically, using the history of observations $\mathcal{D}$ to create a prior over functions. On the other hand, a common choice for acquisition function is the Expected Improvement (EI), which is defined as:

\begin{align}
a(\mathbf{x}|\mathcal{D})=\mathbb{E}\left[\max\left\{ f(\mathbf{x})-y_{\text{min}}, 0\right\}\right]\, 
\end{align}

where $y_{\text{min}}$ is the smallest observed value of $f$.

When using  a GP as surrogate in a BO iteration, we update the posterior after a new configuration has been evaluated. If we define a prior distribution over the GP hyperparameters (hyper-priors), we can estimate a suitable set of these hyper-priors by performing maximum a posteriori estimation (MAP), as explained in Section \ref{gp_hyper_priors}. Therefore, the posterior approximation provided by PFNs sets a novel way to speed-up this process. We use as surrogate a Transformer that outputs a Riemann Distribution and provides a discrete probabilistic output $s_b(\mathbf{x})$ for a bucket $b \in \mathbf{B}$. This allows formulating EI as:

\begin{align}
a(\mathbf{x}|\mathcal{D}) = \sum_{b \in \mathbf{B}} \max\Big\{ {\frac{y_b^{\text{max}}+y_b^{\text{min}}}{2}-y_{\text{min}}} ,0 \Big\} \cdot s_b(\mathbf{x}),
\end{align}

where $y_b^{\text{min}}= \min_{y \in b} y$ and $y_b^{\text{max}}= \max_{y \in b} y$ are the borders of the bucket $b$.


\textbf{Setup of Datasets} We evaluate the performance of our proposed model in the meta-validation and meta-test split of HPO-v3 \citep{}, which contains 16 search spaces with pre-computed evaluations of the performance for different hyperparameter configurations. We ran our method and baselines on all the datasets specified by this meta-dataset and repeat the experiments five times using the five random seeds proposed for starting the HPO algorithms. All the BO evaluations were performed for 10 trials.

\textbf{Setup of Our Model} We use a transformer architecture (Section \ref{gp_hyper_priors}) with 1000. For training, we sampled inputs from an uniform distribution so that the input matches the search space dimensionality. The corresponding target was generated by sampling a function over the prior defined by GP with Mat\'{e}rn 32 kernel and hyperparameters sampled from a gamma distribution as prior. We tuned three hyper-hyperparameters (hyperparameters of the hyperprior): noise, lengthscale and outputscale concentration). The best hyper-hyperparameters were obtained by selecting the combination with the lowest average rank at the 10-th trial. The best yielded hyperprior configuration was: 1) lengthscale concentration: 10, 2) outputscale concentration: 1, 3) noise concentration 0.001. 

\textbf{Setup of Baselines} As baselines we use 1) Random Search \citep{}, a simple yet practical method for HPO, 2) a GP with tuned hyperprior by following the same protocol as for the transformer (and yielding the same best configuration values); 3) DNGO \citep{} a Bayesian Neural Network which uses Bayesian linear regression model to generate a posterior distribution; and  4) BOHAMIANN \citep{}, a Bayesian Neural Networks trained via a stochastic gradient Hamiltonian Monte Carlo. For the BNN, we used the setting proposed by the original authors.

\textbf{Experimental Results}
We show an aggregation of the results for our experimental setup in Figure \citep{fig:mainresults}. Further details on the results per search space are in the Appendix \ref{}. We highlight the close performance of our method (Transformer) compared to the GP and BNN, which is possible to read from the average regret and rank plots. Specially the Crititical Difference diagrams indicate that the difference up to 5 trials is not significant. 


\begin{figure}[htb!]
\centering
\begin{subfigure}[b]{0.58\textwidth}
      \centering
      \includegraphics[width=1.0\textwidth]{iclr2022/bo-plots/regret_and_rank.png}
\end{subfigure} 
%\hfill
\begin{subfigure}[b]{0.41\textwidth}
%\vspace{-7cm}
\includegraphics[width=1.0\textwidth]{iclr2022/bo-plots/cd_diagram_1.png}
\medskip
\includegraphics[width=1.0\textwidth]{iclr2022/bo-plots/cd_diagram_5.png}
\medskip
\includegraphics[width=1.0\textwidth]{iclr2022/bo-plots/cd_diagram_10.png}
\end{subfigure}
 \caption{Left: Comparisons of normalized regret and mean ranks across all search spaces for Random Search (RS), Gaussian Process (GP), Transformer, DNGO and BOHAMIAN. The bounds indicate the 95\% confidence interval. Right: Critical Diagram for showing the significance on ranks via Wilcoxon Test for 1, 5 and 10 trials. }
    \label{fig:mainresults}
    
\end{figure}

==> tabular_cpu_time_spent.tex <==
\begin{tabular}{llllllllll}
\toprule
Transformer CPU &    Transformer GPU & logistic &       GP &      KNN &       BNN & Catboost &       XGB \\
\midrule
0:00:13 &  0:04:23 &  0:09:56 &  0:24:30 &  0:00:34 &  12:04:41 &  2:05:20 &  20:59:46 \\
\bottomrule
\end{tabular}

==> tabular_ece.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
T-Causal &  T-BNN &  T-Meta-GP &  logistic &    GP &   KNN &   BNN &  Catboost &   XGB \\
\midrule
 0.025 &  0.025 &      0.067 &     0.157 & 0.095 & 0.093 & 0.089 &     0.157 & 0.066 \\
\bottomrule
\end{tabular}
